Towards Practical Bayesian Parameter and State Estimation

Joint state and parameter estimation is a core problem for dynamic Bayesian networks. Although modern probabilistic inference toolkits make it relatively easy to specify large and practically relevant probabilistic models, the silver bullet---an efficient and general online inference algorithm for such problems---remains elusive, forcing users to write special-purpose code for each application. We propose a novel blackbox algorithm -- a hybrid of particle filtering for state variables and assumed density filtering for parameter variables. It has following advantages: (a) it is efficient due to its online nature, and (b) it is applicable to both discrete and continuous parameter spaces . On a variety of toy and real models, our system is able to generate more accurate results within a fixed computation budget. This preliminary evidence indicates that the proposed approach is likely to be of practical use.

==> 04system.tex <==
%This section contains the discussion, design and implementation of the inference engine.

%We firstly introduce the language interface of Swift, and then introduce the compiler level optimizations for both memory and computational efficiency. We end this section by illustrating the integrated algorithms.

\name compiles the inference algorithm and the input DPM to a highly optimized C++ target for computation. In this section, we describe the compiler level optimizations for memory efficiency and computational efficiency. Later we introduce the integrated algorithms. All the techniques are extensible for any PPL systems for DPMs.

% \subsection{Syntax}

% Swift uses the syntax of BLOG~\cite{li2013blog} for its conciseness and expressiveness power. We are considering the following sin model described in \cite{erol2013extended}.
% \beq
% 	x_t &=& \sin(\theta x_{t-1}) + v_t, v_t \sim \gauss(0,4) \nn  \\
% 	y_t &=&x_t +w_t, w_t \sim \gauss(0,0.5^2)
% \label{eq:sin_model}
% \eeq

% The corresponding BLOG program for this model is shown below.
% \begin{small}
% %\begin{blogcode}
% \begin{lstlisting}
% random Real theta ~ UniformReal(-1,1);
% random Real x(Timestep t) ~ 
%   if t == @0 then Gaussian(0, 1)
%   else Gaussian(sin(theta * x(prev(t))), 2^2);
% random Real y(Timestep t) ~ Gaussian(x(t), 0.5^2);
% extern Real loadData(Timestep t);
% obs Y(@now) = loadData(@now);
% \end{lstlisting}
% %\end{blogcode}
% \end{small}

% In this program, there is a special type, \texttt{Timestep}, denoting the type of ``time'', namely the iteration number. \texttt{@0} denotes timestep 0 while \texttt{@now} is a special symbol denotes the current timestep. A random variable with an argument of type \texttt{Timestep} will be considered as a dynamic variable, i.e. \texttt{X(t)} is a dynamic variable. Whereas, other variables will be considered static variables or parameters to be estimate, i.e. \texttt{theta} is a parameter. The function \texttt{prev()} is a built-in function for computing the previous timestep, namely $t-1$, which helps Swift to analyze the Markov order of the model. Swift also allows users to write $t-1$ directly but that might lead to incorrect analysis of the model. In this model \texttt{Y} will be observed for each timestep. \texttt{extern} is the key word to declare user-defined C++ function \texttt{loadData()}. 

% With the syntax of BLOG, user could model any complicated dependencies via \texttt{if} and \texttt{case} statement. Swift supports a variety of distributions and built-in functions. Moreover, any external C++ function can be called in Swift, i.e., a user could use their own functions to dynamically load data into Swift.

\subsection{Memory Efficiency}
\textbf{Memory Pre-allocation: }
Memory management is a critical issue for particle filter algorithms since it is often necessary to launch a large number of particles in practice.
%Offline systems (or offline algorithms) records all particles in the history which reduces the maximum number of possible particles. 
Systems that does not manage the memory well will repeatedly allocate memory at run time. For example, in BLOG and Figaro, the inference engine will allocate memory for new particles and erase the memory belonging to the old ones after each iteration. This introduces tremendous overhead since memory allocation is slow.

By contrast, \name will analyze the input model and allocate the minimum static memory for computation: if the user specifies to run $N$ particles, and the Markov order of the input model is $D$, \name will allocate static memory for $(D+1)*N$ particles in the target code. When the a new iteration starts, we utilize a rotational array to re-use the memory of previous particles.

\textbf{Lightweight Memoization: }
In Biips, the compiled target code will sample variables explicitly according to their declaration order in the model. It becomes feasible for Biips since any sorts of condition statements (i.e., if statement) are not supported, which results in a fixed dependency graph. However, the very restricted syntax of Biips is often infeasible for complicated real-world  applications. Notice that adopting an expressive language interface (i.e. syntax of BLOG) might lead to time-varying dependencies between random variables. \name memoizes the value for each random variables already sampled. An example compiled code fragment for the sin model (\ref{eq:sin_model}) is shown below.

\begin{scriptsize}
\begin{minted}{cpp}
class TParticle { public:
// value of x and y at current timestep
  double val_x, val_y;
// flag of whether x/y is sampled
  int mark_x, mark_y; 
}particles[N][DEP]; // particle objects
// getter function of y(t)
double get_y(int t) { 
// get the corresponding particle
  TParticle &part = get_particle(t); 
  // memoization for y(t)
  if(part.mark_y == cur_time) return part.val_y; 
  part.mark_y = cur_time;
// sample y(t), call getter function of x(t)
  part.val_y = sample_normal(
               sin(get_theta() * get_x(t-1)), 0.5);
  return part.val_x; }
\end{minted}
\vspace{-2mm}
\end{scriptsize}

This code fragment demonstrate the basic data structures as well as the memoization framework in the target code. \texttt{N} denotes the number of particles.  \texttt{DEP} is equal to the Markov order of the model plus 1.
In the memoization framework, \name allocates static memory for all the random variables within a particle data structure and generates a flag for each random variable denoting whether it has been sampled or not. Each random variable also has its \emph{getter} function. Whenever accessing to a random variable, we just call its getter function.
In practice, memoization causes negligible overhead.

Memoization also occurs in Figaro and BLOG. However, every random variable in Figaro and BLOG has a string ``name'', and a generic hashmap is used for value storage and retrieval, which brings a great deal of constant factor at run time. 

\textbf{Other Optimizations: } \name also avoids dynamic memory allocation as much as possible for intermediate computation step. 
For example, consider a multinomial distribution. When its parameters change, a straightforward implementation to update the parameters is to re-allocate a chunk of memory storing all the new parameters and pass in to the object of the multinomial distribution. However, this dynamic memory allocation operation is also avoided in \name by pre-allocating static memory to store the new parameters.

\subsection{Computational Efficiency}
\textbf{Pointer References: }
Resampling step is critical for particle filter algorithms since it requires a large number of data copying operations. Note that a single particle might occupy a large amount of memory in real applications. Directly copying data from the old particles to a new ones induce tremendous overhead.

In \name, every particle access to its data via an indirect pointer. As a result, redundant memory copying operations are avoided by only copying the pointers referring to the actual particle objects during resampling
Note that each particle might need to store multiple pointers when dealing with models with Markov order larger than 1. An example compiled code is shown below.

\begin{scriptsize}
\begin{minted}{cpp}
// indirect pointers to the actual particle
TParticles* part_ptrs[N][DEP]; 
TParticle& get_particle(int t) {// rotational array
  return *part_ptr[cur_part][t % DEP]; }
\end{minted}
\vspace{-1.5mm}
\end{scriptsize}

\textbf{Locality: }
Besides using pointer references to reduce the amount of moving data, \name also enhances program locality to speed up re-sampling.
%, when the number of particle becomes large, copying a large number of pointers is also expensive at run-time. To make the process even faster,
In the compiled code, the index of the arrays stores the indirect pointers are carefully designed to take advantage of memory locality when copying. The fragment of code used in resampling step is shown below.

\begin{scriptsize}
\begin{minted}{cpp}
void resample_ptr( int* target,
  TParticle* part_ptr[N][DEP], //storage of  pointers
  TParticle* backup_ptr[N][DEP]) // temporary storage 
{ for (int i = 0; i < N; ++i) {
    // pos: index of particle to copy data from
    int& pos = target_ptr[i];
    // move continuous range of data
    memcpy(backup_ptr[i], part_ptr[pos],
           sizeof(TParticle*)* DEP);  }
  std::memcpy(ptr_temp_memo, backup_ptr,
              sizeof(TParticle*)* DEP * N);}
\end{minted}
\vspace{-1.5mm}
\end{scriptsize}

In the preceding code fragment, the first dimension of the storage array, \texttt{part\underline{ }ptr}, corresponds to the particle index. While the second dimension corresponds to the current iteration. In this case, when copying the pointers during resampling step, all the memory are continuously located in the memory space, which greatly reduces the constant factor at run time.

In our experiment, when dealing with small models where the resampling step takes a large fraction of overall running time, these compiler level techniques helps \name achieve over 250x speedup.

\textbf{Other Optimization: } 
 Notice that the approximation computation in \filter only requires the local data in a single particle and approximation results does not influence the weight of that particle. Therefore, one important optimization specialized for \filter is that \name resamples all the particles prior to the approximation step at each iteration and only updates the approximation distribution for those particle that does not disappear after the resampling step. Notice that it is often the case that a small fraction of particles have significantly large weights. Hence, in practice the overhead due to the $M$ extra samples would be much smaller than the theoretical factor. By contrast, the perturbation step in Liu-West filter must be strictly applied to each particle. Despite the fact that in theory \filter should be $M$ times slower than basic particle filter and Liu-West filter, in our experiment, our implementation of \filter in \name causes merely negligible overhead.

In addition, when computing the weight for each particle, \name also caches the likelihood results for re-use.

\subsection{Algorithm Integration}
Currently \name supports the basic particle filter algorithm, Liu-West filter and \filter. User can specify any of these algorithms as the inference algorithm as well as the number of particles. The Markov order of the input model will be automatically analyzed.

When choosing \filter, \name analyzes all the static parameters in the model and compiled different approximation distributions for different types of random variables. At the current stage, \name supports Gaussian and Mixtures of Gaussian to approximate continuous variables and multinomial distribution for discrete variables. More approximation distributions are under development. For sampling approach, by default \name assumes all the parameters are independent and uses deterministic sampling when possible. User could also ask \name to generate random samples instead. Besides, the number of approximation samples ($M$), the number of mixtures ($K$) for mixtures of Gaussian can be also specified. By default, $M=7$ and $K=10$.


==> makefile <==
MAIN=paper
TENSAKU= tensaku
TEXPARTS= *.tex
FLAGS=-shell-escape -synctex=1 -interaction=nonstopmode

BIBPARTS= BIB/*.bib
# LPR= pspr # or change to 'qpr -q ps3'
# POSTSCRIPT= dvips -P cmz -t letter  #dvips -f
FIGPARTS= FIG/*.fig FIG/*.png
STYPARTS= *.sty
OTHER= dotest makefile README
ALLPARTS= $(MAIN).tex $(TEXPARTS) $(BIBPARTS) $(FIGPARTS) $(OTHER) $(STYPARTS)

# use *this*, to have the svn version within latex
# $(MAIN).pdf: $(MAIN).tex $(TEXPARTS) svnset


$(MAIN).pdf: $(MAIN).tex $(TEXPARTS) 
	pdflatex $(FLAGS) $(MAIN).tex
	bibtex $(MAIN)
	pdflatex $(FLAGS) $(MAIN).tex
	bibtex $(MAIN)
	pdflatex $(FLAGS) $(MAIN).tex

svnset:
	svn propset svn:keywords 'HeadURL LastChangedDate LastChangedRevision LastChangedBy' *.tex
	touch svnset



try: $(MAIN).tex
	pdflatex $(MAIN)

clean:
	\rm -f *.dvi $(MAIN).ps *.bbl *.aux *.log *.blg *.toc all.tar* uu \
	*~ *.bak *.lbl *.brf *.out

spotless: clean
	\rm -f $(MAIN).ps $(MAIN).pdf $(MAIN).svn svnset
	\rm -f final.ps final.pdf final.svn 
	\rm -rf TST

all.tar:
	tar cvfh all.tar $(ALLPARTS)

	# tar cvfh all.tar makefile $(MAIN).tex $(TEXPARTS) $(BIBPARTS) \
	$(FIGPARTS) $(STYPARTS) README


